The Spectral Type of the Ionizing Stars and the Infrared Fluxes of HII Regions

The 20 cm radio continuum fluxes of 91 HII regions in a previously compiled catalog have been determined. The spectral types of the ionizing stars in 42 regions with known distances are estimated. These spectral types range from B0.5 to O7, corresponding to effective temperatures of 29 000-37 000 K. The dependences of the infrared (IR) fluxes at 8, 24, and 160 $\mu$m on the 20 cm flux are considered. The IR fluxes are used as a diagnostic of heating of the matter, and the radio fluxes as measurements of the number of ionizing photons. It is established that the IR fluxes grow approximately linearly with the radio flux. This growth of the IR fluxes probably indicates a growth of the mass of heated material in the envelope surrounding the HII region with increasing effective temperature of the star.

==> maikbibl.tex <==
%
% maikbibl.tex 29.11.2001
%
\documentclass[
aps,%
12pt,%
final,%
notitlepage,%
oneside,%
onecolumn,%
nobibnotes,%
nofootinbib,%
superscriptaddress,%
noshowpacs,%
centertags]%
{revtex4}
\bibliographystyle{maik}
\begin{document}
\selectlanguage{english}
\section*{maik.bst}
\nocite{*}
\bibliography{maikbibl}
\end{document}

